Heuristics2Annotate: Efficient Annotation of Large-Scale Marathon Dataset For Bounding Box Regression

Annotating a large-scale in-the-wild person re-identification dataset especially of marathon runners is a challenging task. The variations in the scenarios such as camera viewpoints, resolution, occlusion, and illumination make the problem non-trivial. Manually annotating bounding boxes in such large-scale datasets is cost-inefficient. Additionally, due to crowdedness and occlusion in the videos, aligning the identity of runners across multiple disjoint cameras is a challenge. We collected a novel large-scale in-the-wild video dataset of marathon runners. The dataset consists of hours of recording of thousands of runners captured using 42 hand-held smartphone cameras and covering real-world scenarios. Due to the presence of crowdedness and occlusion in the videos, the annotation of runners becomes a challenging task. We propose a new scheme for tackling the challenges in the annotation of such large dataset. Our technique reduces the overall cost of annotation in terms of time as well as budget. We demonstrate performing fps analysis to reduce the effort and time of annotation. We investigate several annotation methods for efficiently generating tight bounding boxes. Our results prove that interpolating bounding boxes between keyframes is the most efficient method of bounding box generation amongst several other methods and is 3x times faster than the naive baseline method. We introduce a novel way of aligning the identity of runners in disjoint cameras. Our inter-camera alignment tool integrated with the state-of-the-art person re-id system proves to be sufficient and effective in the alignment of the runners across multiple cameras with non-overlapping views. Our proposed framework of annotation reduces the annotation cost of the dataset by a factor of 16x, also effectively aligning 93.64% of the runners in the cross-camera setting.

==> Methodology.tex <==
\section{Methodology}
\subsection{Annotation Procedure}
\textbf{Annotating videos.} Video annotation is similar as image annotation. It involves mainly two steps: i) Extracting the frames from videos, ii) Annotation of individual frames.

\textbf{Manually annotating runners.} The main object of interest here is the runner. We used the basic bounding box annotation around the runners. The bibId of the runner is used as the label. The label is manually added by the annotator. Firstly, a runner is selected, then we try to find a frame in which the runners bibId is clearly visible. We then move back to the frame number where the runner is visible for the first time in the camera. We start putting bounding boxes around the runner in all the frames in which he/she is visible, until the runner leaves the camera frame. We followed runner-wise annotation instead of frame-wise annotating all objects of interest.

\subsection{Creating sample dataset}
The large size of the dataset makes it difficult for validating the experiments. Hence, a sample dataset is required, that is a true representative of the actual dataset. A smaller version of the dataset is created by down-sampling the original one and covering different scenarios present in different video locations. 

\textbf{Assigning Scores to locations.} Firstly, variations in different scenarios is analyzed at all the recording locations. The scenarios are divided into following five categories: \textit{i) resolution, ii) lighting condition, iii) recording angle, iv) occlusion, v) number of crowded videos}. Different scenarios and their score distribution is shown in table \ref{table:scoreDistribution}.

\begin{table*}[ht]
\begin{center}
\begin{tabular}{| p{1cm} | p{2cm} | p{2cm} | p{5cm} | p{2cm} | p{3cm} |}
\hline
         \textbf{Scores} & \textbf{Lighting} & \textbf{Resolution} & \textbf{Recording Angle} & \textbf{Occlusion} & \textbf{\# Crowded Videos}\\\hline
         1 & Very poor & Very poor & Front+Side+Static+Upside-Down & Very high & Very large\\
         2 & Poor & Poor & Side & High & Large\\
         3 & Moderate & Moderate & Front+Downside+Static & Moderate & Moderate\\
         4 & Good & Good & Front+Side & Low & Less\\
         5 & Very good & Very good & Front & Very low & Very less\\
\hline
\end{tabular}
\end{center}
\caption{Different scenarios and their score distribution. All video locations are analyzed and penalized as per the scenarios of the video recording at that location. A location score is the sum of scores in different scenarios.}
\label{table:scoreDistribution}
\end{table*}

The total score of a location is the sum of scores in individual categories of different scenarios. Location score $S_{location}$ is given by,

$S_{location} = S_{lighting} + S_{resolution} + S_{recordingAngle} + S_ {occlusion} + S_{noOfCrowdedVideos}$ ,

Consider an example location 'X' having videos recorded in poor lighting conditions(2), with good resolution(5), view of recording is front(5), occlusion is moderate(3) \& number of videos having too many crowded runners is moderate(3), then the total score is 
$S_{X} = 2 + 5 + 5 + 3 + 3 =18$.

All the 42 recorded locations are given scores s = [0,5] in each of the above mentioned categories, refer to \ref{apdx:ksTest}. The frequency vs score distribution of the entire dataset is shown in figure \ref{fig:freqScoreDistribution}. There are total 16 different score values ranging from 8 to 24. Higher scores implies better recording scenarios in videos.

\begin{figure}[ht]
                \centering
                \includegraphics[width=\linewidth]{latex/images/Methodology/SampleDataset/FrequencyScoreDistribution.png}
                \caption{Score distribution of the entire dataset. Frequency represents the number of locations with a given score.}
                \label{fig:freqScoreDistribution}
\end{figure}

\textbf{Kolmogorov-Smirnov (KS) Test.} The Kolmogorov–Smirnov test is used to test whether two underlying one-dimensional probability distributions differ.

The two-sample K–S test is one of the most useful and general non-parametric methods for comparing two samples, as it is sensitive to differences in both location and shape of the empirical cumulative distribution functions of the two samples.

For larger sample sizes, the approximate critical value $D_{\alpha}$ is given by the equation,

$D_{\alpha } = c{(\alpha)}\sqrt{\frac{n_{1} + n_{2}}{n_{1}n_{2}}}$,\newline

where, $n_{1}$ and $n_{2}$ are the sample sizes of the two distributions and $\alpha$ and $c{(\alpha)}$ are the coefficients given by table mentioned ~\cite{kstest}. More information can be found in Appendix \ref{apdx:ksTest}.


\textbf{How to select locations?} To select desired number of locations for the sample dataset, we use Kolmogorov-Smirnov Test for distribution similarity matching. The score distribution of both sample dataset and the original dataset is assumed to be gaussian. Here, we randomly select 6 scores out of total 16, and matches the similarity of the selected scores with the original dataset scores. The K-S test calculates the distance between the two distributions, and the sample distribution of the randomly selected 6 score values, having the minimum distance from the actual data distribution is selected.

\begin{figure}[ht]
                \centering
                \includegraphics[width=\linewidth]{latex/images/Methodology/SampleDataset/DistributionMatching.png}
                \caption{The graph shows the probability distribution of the scores of the original and the sampled dataset. The sample score values [11, 15, 16, 17, 19, 23] is having distribution that fits nicely with the actual dataset score distribution.}
                \label{fig:distributionSimilarity}
\end{figure}

We selected score values [11, 15, 16, 17, 19, 23] for the sample dataset. The distribution of the selected values and the original dataset is shown in figure \ref{fig:distributionSimilarity}. Now, 6 locations having these scores are selected. In all, 60 videos are collected, corresponding to top 20 and middle 3 runners. It is made sure that all these runners appears in all the 6 sampled video locations. It is necessary for the validation of the cross-camera alignment. However due to unavoidable circumstances, there can be runners other than the selected ones, appearing in each sampled location.


\subsection{Webscraping the data}
\subsection{Creating Tool for Inter-Camera Alignment}
